Bouncing threads for infinitary and circular proofs

We generalize the validity criterion for the infinitary proof system of the multiplicative additive linear logic with fixed points. Our criterion is designed to take into account axioms and cuts. We show that it is sound and enjoys the cut elimination property. We finally study its decidability properties, and prove that it is undecidable in general but becomes decidable under some restrictions.

==> decid-intro.tex <==
%\TODO{Dans toute cette section, il ne sera pas parlé des occurrences.}
\subsection{An operational approach to threads}\label{sec:stack}

In this section, we will explicit how threads can be recognized by a specific deterministic pushdown automaton reading only the weight of a pre-thread.
This will allow us to define the \emph{height} of a thread and the notion of \emph{constraint stack}.

Let $\Athread$ be the deterministic pushdown automaton described in Fig. \ref{fig:Athread}, on alphabet $\Sigma=\{l,r,i, \bar{l},\bar{r},\bar{i},A,C, W\}$ and stack alphabet $\Gamma=\{l,r,i,\bot\}$ where $\bot$ is the empty stack symbol. 
%The \buchi condition is defined on transitions, \buchi transitions are represented by double arrows. This means that a run is accepting if and only if a \buchi transition is taken infinitely many times.
The transitions are labelled ``$(a,\gamma) \mid \tau$'', where $a\in\Sigma$ is the input letter, $\gamma\in\Gamma$ is the topmost stack symbol, and $\tau$ is the action performed on the stack (no action if $\tau$ is not specified). If no stack symbol is specified, the stack is left unchanged. Symbol $x$ stands for an element in $\{l,r,i\}$. No acceptance condition is specified, meaning that any run is accepting. Only the absence of an available transition can cause the automaton to reject its input, for instance reading $l$ with topmost stack symbol $r$ in state $\uparrow$.
The transition marked with a double arrow corresponds to the visible part of the thread.

\begin{figure}[t]
\centering
\begin{tikzpicture}[shorten >=1pt,node distance=3cm,on grid,auto,initial text=,
every state/.style={inner sep=0pt,minimum size=6mm}, every loop/.style={min distance=.5cm, looseness=10}]

\node[state,initial] (up) {$\uparrow$};
\node[state, right=of up] (down) {$\downarrow$};
\path[->]
	(up) edge[loop below,double] node{$(x,\bot)$} ()
	edge[loop above] node{$\begin{array}{c}(x,x)\mid\pop()\\W\end{array}$} ()
	edge[bend left] node {$A$} (down)
	(down) 	edge[loop above] node{$\begin{array}{c}(\bar{x},\gamma)\mid\push(x)\\W\end{array}$} ()
	edge[bend left] node {$C$} (up)
	;
\end{tikzpicture}
\caption{The deterministic pushdown automaton $\Athread$}
\label{fig:Athread}
\end{figure}

\begin{lemma}
Let $t$ be a pre-thread. Then $t$ is a thread if and only if $\weight{t}$ is accepted by $\Athread$.
\end{lemma}

\begin{proof}
The constraints on the stack match the grammar from Def. \ref{def:thread}. %The B\"uchi condition ensures that the visible weight is infinite.
\end{proof}

The stack of $\Athread$ will be referred to as the \emph{constraint stack}.



==> introduction.tex <==

\input{new-intro}
%%
\section{Introduction}\label{sec:Intro}
%%
Infinitary (non-wellfounded) and circular proof systems have received much 
attention in recent years.
Such proof systems allow non-wellfounded proof trees and impose some global 
validity condition in order to ensure soundness. Typically, it requires that
every infinite branch is supported by some \emph{thread} which traces some 
formula in a bottom-up manner and witnesses infinitely many progress points of 
a coinductive property. 

Unfortunately, existing notions of validity impose a quite limited use of cuts 
in non-wellfounded proofs and many proofs that could be accepted as valid
are rejected.
This paper introduces a new validity condition for \muMLLi,
the infinitary proof system for multiplicative linear logic with fixed 
points. This criterion generalizes the existing one, taking inspiration from 
Geometry of Interaction, enriching the structure of threads and relaxing their 
geometry: bouncing threads can leave the branch they validate and ``bounce''
({\it i.e.}\ change direction, moving upward but also downward along proof 
branches) on axioms and cut rules.

We define a new \emph{bouncing} validity condition in the multiplicative 
fragment and show that the obtained proofs enjoy cut elimination.
This new validity condition is undecidable but can be decomposed into an
infinite hierarchy of decidable conditions. Moreover, it naturally extends
to a validity condition ensuring cut elimination for the multiplicative
and additive fragment.
\TODO{en rajoutant quelques citations le paragraphe ci dessus est suffisant pour faire une intro}

\emph{Organization of the contributions.}
In Section~\ref{sec:ProofSystemMuMLL} we recall the basic definitions for the non-wellfounded proof system \muMALLi.
We then define, in \cref{sec:CutElimRules} the cut-elimination procedure. In \cref{sec:ValiditeMuMLL}, we introduce our new bouncing validity 
condition, and show in \cref{sec:muMLLCutElimThm} that it guarantees soundness of the system and productivity of the cut-elimination procedure. We finally study in \cref{sec:decid-body} the decidability of our criterion in the multiplicative case.

%
%Fixed point theory has proved to be a valuable tool in computer
%science, in particular for reasoning formally about software systems.
%% Its explicit uses may be traced back to the first formal
%% semantics of programming languages in the late 
%% 1960s~\cite{sangiorgi2009origins} and
%It is pervasive in programming language semantics,
%concurrency, automata theory and software verification techniques.
%
%\textcolor{gray}{A notable early use of fixed point theory is found in the work of Park % 1970s
%on fairness properties of software systems, which involved a rich use of 
%greatest fixed points and alternating least and greatest fixed points;
%Park's expertise was instrumental when, together with Milner,
% he came up with the notion of coinduction~\cite{sangiorgi2009origins}.
%As part of the increasing use of fixed points in computer science,
%logics featuring fixed points, generally referred to as \emph{$\mu$-calculi},
%were developed and studied~\cite{pratt1981decidable,kozen83tcs}.
%Decades later, fixed points are used in various specification languages,
%e.g.\ to specify temporal or spatial properties of program executions.
%Fixed points are also present in most programming languages as
%recursive types. More interestingly, the Curry-Howard correspondence,
%which allows to view proofs as programs and formulas as types,
%has been extended in various ways to encompass fixed point types,
%e.g.\ in System F extended with least and greatest fixed point 
%types~\cite{mendler91apal}, % matthes98csl
%in Coq's calculus of (co)inductive constructions~\cite{gimenez98icalp},
%and in typing disciplines for functional reactive programming
%based on the linear-time $\mu$-calculus~\cite{cave2014popl}.}
%
%%% Quelques références sur FRP
%% https://dl.acm.org/citation.cfm?id=2535881
%% https://dl.acm.org/citation.cfm?id=3209148
%% https://dl.acm.org/citation.cfm?id=2500588
%
%% \paragraph{Inductive and coinductive predicates / Logics with least and greatest fixed points}
%% Reactive systems being pervasive, coinduction has been for the last 20/30/? years a major topic in computer science. This allows both reasoning on infinite behaviours and modelling of infinite data such as streams, infinite trees or more refined coinductive objects such as fair schedulers\todo{ref?}.
%% 
%% In this field, logical formalisms encompassing inductive and coinductive predicates have been successful in expressing elaborated properties while amenable to a formal and mecanicle treatment. Among them, logics with least and greatest fixed points have been rising in the last decades.
%
%%Proof systems for fixed point logics can naturally be obtained by taking 
%%(co)induction rules that closely reflect fixed point theorems,
%%e.g.\ Knaster-Tarski's characterization of least fixed points as least 
%%pre-fixed points.
%%This is the basis of Kozen's famous axiomatization~\cite{kozen83tcs} of the $\mu$-calculus.
%\gray{When building finitary proofs for logics with fixed points, one has to identify (co)invariants
%which may be significantly more complex than the property to establish --
%a phenomenon that students encounter when learning to prove
%properties by induction on natural numbers.}\TODO{reformuler rapidement} An alternative to these
%explicit (co)induction rules is to consider proof systems featuring
%non-wellfounded derivation trees: this makes it possible to reason on
%fixed points by unfolding them, possibly infinitely often. However, the soundness of such systems requires a global
%\emph{validity} condition that ensures that some progress is made along
%each infinite branch. Consider for instance the following (regular) infinite
%derivation, which repeatedly applies the fixed point unfolding rule $\rsigma$
%where $\sigma \in \{\mu,\nu\}$:
%\\[2ex] \null\hfill $\scalebox{.9}{\begin{prooftree}
%  \Hypo{\vdash \sigma X.\orig{introa}X}
%  \Infer{1}[\rsigma]{
%    \vdash \sigma X.X
%    \begin{tikzpicture}[remember picture,overlay]
%      \node[inner sep=0pt,outer sep=0pt] (introb) {\ensuremath{}};
%      \draw [->,>=latex] (introa.north) .. controls +(35:1.5cm) and +(0:1.5cm) .. (introb.west);
%    \end{tikzpicture}
%  }
%\end{prooftree}}$ \hfill\null \\[2ex]
%The system would be unsound if this derivation were declared valid for both
%$\sigma=\nu$ and $\sigma=\mu$. However, the validity condition should also
%accept the derivation when $\sigma=\nu$ since $\nu X.X \equiv \top$ (a tautology).
%In the case of arithmetic, this style of reasoning is 
%akin to proofs by infinite descent rather than by induction, and has been
%formally studied in infinitary sequent calculus by Brotherston and
%Simpson~\cite{brotherston11jlc}.
%For propositional $\mu$-calculus, several such infinitary deduction systems
%have been proposed~\cite{kozen83tcs,streett89ic,janin95mfcs,dax06fsttcs}.
%Because they are easier to work with than the finitary proof systems (or 
%axiomatizations) based on Kozen-Park (co)induction schemes, they are often 
%found in completeness arguments for such finitary systems~\cite{kozen83tcs,walukiewicz93lics,walukiewicz95lics,walukiewicz00ic,kaivola95concur,doumane16lics}. They are also better suited for automated
%reasoning~\cite{streett89ic,dax06fsttcs}.
%
%In both uses, regular derivation trees play a particular role; such proofs, that we call \emph{circular}, can be represented by a finite tree with back-edges. 
%%Circular proofs are those infinitary proofs that can be easily represented and algorithmically processed in a finite time.%finitely presented by means of cycles in the construction of the derivation tree.
%%\todo[inline]{peut être déplacer ailleurs, mais garder une mention dans l'intro de ce qu'est circulaire pour que le lecteur ne termine pas l'intro sans le savoir...}
%% There are many other uses of infinite (or regular) derivations,
%% \eg
%% circular proofs~\cite{santocanale02fossacs} as a system for representing morphisms in $\mu$-bicomplete categories \cite{santocanale02ita,santocanale02jpal},
%% to study the relationship between
%% induction and infinite descent in first-order 
%% arithmetic~\cite{brotherston11jlc},
%% to generate invariants for program verification in separation
%% logic~\cite{brotherston14sas},
%% or as an intermediate between ludics' designs and proofs in
%% linear logic with fixed points~\cite{baelde15csl}.
%
%On the other end of the Curry-Howard correspondence, 
%one finds programming languages equipped with 
%(co)recursion constructs whose typing naturally reflects the Kozen-Park 
%(co)induction rules~\cite{mendler91apal,cave2014popl}.
%Writing programs in these systems may be difficult, as it involves
%coming up with complex (co)invariants. These difficulties are only
%partially lifted through the use of guarded 
%(co)recursion~\cite{gimenez98icalp} or sized types~\cite{abel2007mixed}
%in Coq or Agda respectively.
%Furthermore, (co)recursion involves a suspended computation which makes it 
%difficult to analyze the behavior of a program.
%As an alternative, one could naturally consider infinitary (or circular)
%programs, equipped with a global validity condition ensuring that
%they behave well -- in particular that they are terminating, or productive
%for inhabitants of coinductive types.
%There is surprisingly little work following this approach\footnote{
%  We note the work of Hyvernat~\cite{hyvernat2014lmcs} whose use of 
%  size-change termination could be seen as a form of validity checking.
%  It would be interesting to develop this work from a Curry-Howard 
%  perspective to properly compare it with our style of infinitary
%  proof systems.
%}, and
%foundations are missing.
%This can be understood from the fact that the aforementioned
%infinitary proof systems for fixed point logics are all cut-free; hence,
%the role of the validity condition in (syntactic) cut-elimination remains
%unclear from these works. This shortcoming has been addressed first by Santocanale
%and Fortier: in~\cite{fortier13csl} they consider an infinitary sequent
%calculus for purely additive logic, featuring cuts and an extended
%notion of validity, and they show that cuts can be eliminated from valid
%proofs -- in that setting, cut-elimination is not terminating but productive,
%and converges to a (valid) cut-free derivation.
%A key insight of this work is that the same validity condition that ensures
%soundness in infinitary proof systems also ensures the productivity of 
%cut-elimination.
%The result has been generalized later to the multiplicative and additive linear
%logic, at the cost of a more complex argument, by three authors of the present
%paper~\cite{BaeldeDS16}.
%Through these syntactic cut-elimination results, infinitary proofs for
%the multiplicative-additive $\mu$-calculus \muMALL are given a computational
%content, which is an important first step towards an interesting Curry-Howard
%correspondence for that logic.
%
%% Non-wellfounded proof systems were investigated mostly in cut-free systems. There is a historical reason for this, notably the fact that they served a concrete artifact to describe models and were used in completeness results based on proof-search methods (à la Schütte).
%
%% TODO
%% Explain characteristics of the validity criterion: validating a proof requires that each of its infinite branches has to be supported by a thread, that is a sequence of (sub)formulas such that, roughly, a coinductive is unfolded infinitely often along the branch see figure~\ref{cite-example-validity}:
%% - $\nu X.X$ / $\nu X. X\tensor X$
%% - N= mu X. 1+X, ... zeroes = 0:: zeroes -> both examples?
%
%\medskip
%
%In the present paper, we address one general limitation of the
%previous works on cut-elimination for infinitary sequent calculi.
%%
%% In~\cite{BaeldeDS16}, only atom-free logic was considered and the logic
%% therefore admits an axiom-elimination theorem. In the present work, a first contribution will be to provide a proper treatment of the axiom rule in cut-elimination.
%%
%In \cite{fortier13csl,BaeldeDS16}, the validity condition is based on the 
%existence of \emph{threads} that trace formulas through infinite branches,
%and witness infinitely many progress points in the form of $\nu$-unfoldings.
%This notion is adapted from cut-free infinitary deductive systems for 
%propositional $\mu$-calculus, and it barely takes cuts into account, simply
%requiring that threads properly follow formula occurrences from conclusion
%to premisses of cut rules.
%%
%These \emph{straight} threads fail to reflect a lot of the transformations
%that a proof will go through in cut elimination. Although straight validity is 
%preserved in cut reductions, it is not the case for cut-expansion which may break validity.
%As a result, straight validity rejects several sound proofs for which cut
%elimination would hold.
%Consider for instance the following derivation:
%\\[2ex] \null\hfill $\scalebox{.9}{\begin{prooftree}
%  \Infer{0}[\rax]{\vdash \tikzmark{ad3}\nu X.X, \mu X.X\tikzmark{ad4}}
%  \Infer{1}[\rmu]{\vdash \tikzmark{ad2}\nu X.X, \mu X.X\tikzmark{ad5}}
%  \Hypo{\vdash \nu X.\orig{introA}X\tikzmark{ad7}}
%  \Infer{1}[\rnu${\times}2$]{\vdash \nu X.X\tikzmark{ad6}}
%  \Infer{2}[\rcut]{
%    \vdash \tikzmark{ad1}\nu X.X
%    \begin{tikzpicture}[remember picture,overlay]
%      \node[inner sep=0pt,outer sep=0pt] (introB) {\ensuremath{}};
%      \draw [->,>=latex] (introA.north) .. controls +(25:3cm) and +(0:6cm) .. (introB.west);
%    \end{tikzpicture}
%  }
%\end{prooftree}
%  \begin{tikzpicture}[overlay,remember picture,-,line cap=round,line width=0.1cm]
%    \draw[rounded corners, smooth=2,red, opacity=.25] ($(pic cs:ad1)+(-.1cm,.1cm)$) to ($(pic cs:ad2)+(.1cm,-.2cm)$)to ($(pic cs:ad3)+(-.1,.2cm)$) to($(pic cs:ad4)+(-.2cm,.2cm)$) to($(pic cs:ad5)+(-.2cm,0cm)$) to($(pic cs:ad6)+(-.1cm,0cm)$) to($(pic cs:ad7)+(-.1cm,0cm)$) ;
%  \end{tikzpicture}}
%$
% \hfill\null \\[2ex]
%It is not valid according to straight threads. However,
%after reducing twice the cut in each repetition of the cycle, it yields
%the previous example derivation for $\sigma=\nu$. \TODO{Reviewer 2: detail this example: why are two $\nu$-unfoldings needed ? can we explicit the cut elimination steps ? Explain why straight threads reject it.}
%In order to fix this, and accept our derivation as valid, it is natural
%to consider extending the validity criterion to threads that trace formulas 
%more richly in derivations. For instance the red thread in the example above will witness the validity of this proof. This idea will be our guiding principle in 
%designing a relaxed validity condition where threads can ``bounce'' on axioms 
%and cuts to travel up and down in derivations.
%As it turns out, this modest extension of the validity condition
%will result in surprisingly complex issues.
%
%%It does not take into account the fact that, in presence of the axiom rule,
%%the $\rcut/\rax$-reduction case where a cut and an axiom inferences cancel each other. Considering the axiom naturally raises a question about validity which leads us to extend relax the validity condition. Indeed, while validity ensures cut-elimination, it is natural to wonder how robust our validity condition is with respect to cut transformations. When considering cut-reduction or finitary cut expansions, validity is preserved, but when considering $\omega$-chains of cut expansions one easily sees that validity may be lost: a validating thread can be broken into piece as the following example shows:
%
%%In the above example, the problem is that on the cut-expanded proof, the infinite branch contains \defname{no} infinite thread and therefore cannot be validated. Indeed, cut-expansion threads slice the thread into pieces and, at the limit, no infinite thread remains.
%%We interpret this as a confirmation that the original criterion does not deal well the interaction between axiom and cut inferences.
%%As a consequence, the validity condition introduced in CSL rejects many proof objects which could be considered as valid asthey are productive and perfectly sound.
%
%%However, one can easily trace the original thread of the cut-free proof in the resulting proof: each cut-expansion step introduces a detour in the thread which goes up to axiom inferences and then down to cut inference and then up again. This idea will be our guiding principle in designing a relaxed validity condition: threads can make detours through axioms and cuts and travel up and down in the proof tree.
%
%From the Curry-Howard perspective, considering more relaxed validity criteria is an interesting challenge as it may result in richer computational behaviours:
%more proofs means more programs.
%
%\TODO{Insist on the fact that we do have more programs, in particular it does not contradict the cut-elimination result (in response to reviewer 1), since cut elimination can produce non-regular straight proofs from regular bouncing ones. Give a Coq example if possible. Also explain link with GOI clearly. Insist also on the other new contribution: the treatment of axioms.}
%
%A validity criterion should satisfy three important properties:\\
%i) At the {proofs level}:  guarantee cut elimination.\\
%ii) At the {semantic level}:  guarantee the truth of the formulas they prove.\\
%iii) From a {practical point of view}, we would like the criterion to be decidable. 
%We meet the first two requirement; unfortunately we show that our
%criterion is only recursively enumerable.

%\paragraph{Contributions}
%\textcolor{gray}{(this will change) In the present paper, we focus on the multiplicative case, \muMLLi, and address the first two requirements: we prove our {\it Hauptsatz}, a cut-elimination theorem for \muMLLi non-wellfounded derivations validated by the bouncing condition. On the way to the cut-elimination result, we establish a soundness result. 
%The restriction to multiplicative fragment is actually for keeping the presentation simple, since we can add the additives and lift our cut-elimination result to \muMALLi: although this is beyond the scope of the present paper we provided a treatment of the additives in Appendix~\ref{app:Additives}.
%The third requirement is actually not met: the weakly bouncing validity condition is not decidable in general. However we can decompose the bouncing validity condition into a hierarchy of decidable validity conditions. This result will be presented in a forthcoming paper and we shall simply discuss its consequences in the present paper\footnote{We refer the reader to a long version of the paper containing the (un)decidability results and proofs~\cite{bouncing19long}.}.
%}


% from various perspectives:
%* Many productive proofs are not valid
%* Sound Derivations 

%3) Applications to Natural deduction.

%\paragraph{Statement of cut-elimination in an infinitary setting.}
%In a finitary setting, the cut-elimination result is usually stated as follows:
%“Every proof can be reduced after a finite number of steps to a cut-free proof”.
%In an infinitary setting, this result obviously  does
%not hold.
%Actually, what we need to establish it not the termination of the cut-elimination procedure, but its \textbf{productivity}. This property means that every finite prefix of the result can be computed in a finite number of steps.

%The other particularity of cut-elimination in an infinitary setting comes from the validity condition. If productivity guarantees that we obtain a pre-proof at the limit of the cut-elimination procedure, nothing says that it is indeed a proof. We will show in this chapter that the pre-proof obtained by cut elimination satisfies the validity condition, we call the result the \textbf{validity preservation}.
%The productivity being strongly based on the validity of the proof, the validity preservation result is of great importance when we consider higher-order functions, since the result of cut-elimination may be itself used as a function. 

%Finally, as usual with infinitary reductions it is not the case that all reduction sequences converge:
%for instance, one could reduce only deep cuts in a proof, leaving a cut untouched at the root. 
% We avoid this problem by reducing bottom-most cuts only, that is we consider a form of head reduction.





%Even though this is fine in absence of atomic formulas, it hides some of the issues related to the interaction between cuts and axioms in sequent proofs. Indeed, when following up a thread and reaching a formula $A$ in a axiom $\vdash A,A^\perp$ immediately above a cut, the occurrence of $A$ is bound to be identified to the cut-formula  $A$ in the other premiss of the cut from which the thread could continue its path upwards in the pre-proof which is not allowed in our criterion.
%
%blabla cut-reduction/GoI. 



%\paragraph{About the proof.}




%In contrast to~\cite{BaeldeDS16}, we provide 
%in the present paper a treatment of the axiom rules and therefore we have to 
%generalize significantly the proof transformations considered in the 
%cut-elimination process as well as the notion of multicut inference which is 
%used to carry the cut-elimination process; this is done in
%\cref{sec:CutElimRules}.
%
%  which relies on enriching the structure of threads and relaxing their geometry: bouncing threads can move upward but also downward in the proof and they can bounce ({\it ie} change direction) on axioms and multicut rules.
%
%\Cref{sec:muMLLCutElimThm} is then dedicated to proving cut elimination for 
%\muMLLi with our new validity condition.
% [David] pas sûr de trouver ça très important pour être mentionné ici
% In our way to do so, we also prove soundness of this proof system.
%We conclude in \cref{sec:conclusion} by providing directions for future work
%and discussing our extended validity condition and results.
%In particular,
%we mention other results establishing that the bouncing criterion is 
%undecidable in general but can be decomposed into a hierarchy of decidable 
%conditions.
%We also describe how our cut elimination result for \muMLLi
%can be lifted to \muMALLi, which is detailed in \cref{app:Additives}.
%Three appendices provide additional material for the reviewers on
%the cut elimination rules (\cref{app:CutElimRules}), the cut-elimination proof for
%\muMLLi (\cref{app:muMLLCutElimThm}) and its extension to the additives (\cref{app:Additives}).
%}
%% The following Section~\ref{sec:DecUndec} investigates decidability issues related to bouncing validity and proves two results:
%% (i) the general bouncing criterion is already undecidable in the
%% multiplicative circular fragment, %  (where proof are unfoldings of finite graphs)
%% %
%% %
%% %the general bouncing criterion on circular ({\it ie} regular) \muMLLi proofs is proven to be undecidable by reducing the halting problem of Minsky machines to deciding validity of bouncing circular multiplicative proofs and 
%%  (ii) on the other hand we show that the condition can be decomposed into a hierarchy of decidable validity conditions.
%% In Section~\ref{sec:Additives}, we extend the criterion to additives and show cut elimination in this more general setting.
%% %to integrating the additive connective to our picture which is quite involved 
%% %in the bouncing-thread setting additives are more involved
%% %because bouncing threads interact with additive contraction and as such the straightforward generalization of the validity condition of Section~\ref{sec:ValiditeMuMLL} fails to ensure cut-elimination. 
%First, we restrict our attention to MLL in which the cut-elimination and sequent proofs are well-known to enjoy better property (think, for instance, of the theory of proof nets). 


==> macros-types.tex <==
%%% encodage et langue
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{framed} %barres vertivales
\usepackage{wrapfig} %figures entourées de texte
\usepackage{todonotes}
\presetkeys{todonotes}{fancyline, color=orange}{}
\usepackage{stmaryrd}
\usepackage{amsfonts,amstext,amsmath,amssymb}
\usepackage{thmtools,thm-restate}
\usepackage{cleveref}
\newcommand{\para}[1]{\smallskip\noindent\emph{#1}.\xspace}

\def\savespace{\vspace{-.5cm}}

\newcommand{\restatablelemma}[2]{
  \expandafter\newcommand\csname statelemma#1\endcsname{#2}
  \begin{lemma}\label{#1}
    \expandafter\csname statelemma#1\endcsname{}
  \end{lemma}
}
\newcommand{\restatelemma}[1]{
  \begin{claim}[\cref{#1}]
    \expandafter\csname statelemma#1\endcsname{}
  \end{claim}
}

\newcommand{\restatableproposition}[2]{
  \expandafter\newcommand\csname stateproposition#1\endcsname{#2}
  \begin{proposition}\label{#1}
    \expandafter\csname stateproposition#1\endcsname{}
  \end{proposition}
}
\newcommand{\restateproposition}[1]{
  \begin{claim}[\cref{#1}]
    \expandafter\csname stateproposition#1\endcsname{}
  \end{claim}
}

\newcommand{\restatabletheorem}[2]{
  \expandafter\newcommand\csname statetheorem#1\endcsname{#2}
  \begin{theorem}\label{#1}
    \expandafter\csname statetheorem#1\endcsname{}
  \end{theorem}
}
\newcommand{\restatetheorem}[1]{
  \begin{claim}[\cref{#1}]
    \expandafter\csname statetheorem#1\endcsname{}
  \end{claim}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tikz}
\usetikzlibrary{positioning,calc,arrows,shapes}
\usetikzlibrary{automata}
\usepackage{pifont}
\usetikzlibrary{tikzmark,decorations.pathreplacing}
\usepackage{ebproofs}


\newcommand{\TODO}[1]{\textcolor{red}{[TODO #1]}}
%pour cacher les \TODO, décommenter la ligne ci-dessous
%\renewcommand{\TODO}[1]{}

\newcommand{\Frozen}{\mathit{Frozen}}

\long\def\hide#1\endhide{}

\newcommand{\psd}[3]{(#1,#2,#3)}
% polices
\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\F}[1]{\mathfrak{#1}}
\newcommand{\BB}[1]{\mathbb{#1}}
\newcommand{\BF}[1]{\mathbf{#1}}
\newcommand{\RM}[1]{\mathrm{#1}}
\newcommand{\SF}[1]{\mathsf{#1}}
\newcommand{\IT}[1]{\mathit{#1}}
\newcommand{\TT}[1]{\mathtt{#1}}
\newcommand{\net}{}
\newcommand{\switch}{\C}

\newcommand{\fl}[1]{\mathrm{FL}(#1)}

\newcommand{\dbot}{\raisebox{0.05em}{\rotatebox[origin=c]{90}{$\models$}}}
\newcommand{\Aax}{\mathsf{A}}
\newcommand{\Ccut}{\mathsf{C}}
\newcommand{\Wwait}{\mathsf{W}}
% ensembles spécifiques
% premisses d'une inférence de conclusion ...
\def\prem#1{\mathsf{premiss}(#1)}
\newcommand\defeq{\triangleq}
\makeatletter
\newcommand{\bigpole}{%
  \mathop{\mathpalette\bigp@rp\relax}%
  \displaylimits
}

\newcommand{\bigp@rp}[2]{%
  \vcenter{
    \m@th\hbox{\scalebox{\ifx#1\displaystyle2.1\else1.5\fi}{$#1\independent$}}
  }%
}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\makeatother

%%
% utilisation:
% \todoAS{bla bla}
% ou \todoAS[inline]{bla bla}
    %\newcommand\quoi[1]{\todo[color=orange!60,inline]{#1}} 
    \newcommand\todoAS[2][]{\todo[color=blue!60,#1]{Alexis: #2}} 
    \newcommand\todoAD[2][]{\todo[color=red!60,#1]{Amina: #2}} 
    \newcommand\todoDB[2][]{\todo[color=yellow,#1]{David: #2}} 
    \newcommand\todoGJ[2][]{\todo[color=green!60!black,#1]{Guilhem: #2}}
%pour cacher les todo, décommenter la ligne ci-dessous
\renewcommand{\todo}[2][]{}

%%
% Pour les back-edges:
\newcommand{\point}[3]{
  \begin{tikzpicture}[remember picture,overlay]
    \node[inner sep=0pt,outer sep=0pt] (#2)  {\ensuremath{#3}};
    %\coordinate(R) at (0,0);
    \draw [->,>=latex] (#1.north) .. controls +(60:2cm) and +(-30:3cm) .. (#2.east);
  \end{tikzpicture}\;
}
\newcommand{\orig}[2]{\begin{tikzpicture}[remember picture]\node[inner sep=0pt,outer sep=1pt] (#1)  {\ensuremath{#2}};\end{tikzpicture}}
\newcommand{\destgauche}[3]{
  \begin{tikzpicture}[remember picture,overlay]
    \node[inner sep=0pt,outer sep=0pt] (#2)  {\ensuremath{#3}};
    %\coordinate(R) at (0,0);
    \draw [->,>=latex] (#1.north west) .. controls +(120:3cm) and +(200:3cm) .. (#2.west);
  \end{tikzpicture}\;
}
\newcommand{\destdroite}[3]{
  \begin{tikzpicture}[remember picture,overlay]
    \node[inner sep=0pt,outer sep=0pt] (#2)  {\ensuremath{#3}};
    %\coordinate(R) at (0,0);
    \draw [->,>=latex] (#1.north east) .. controls +(60:3cm) and +(-20:3cm) .. (#2.east);
  \end{tikzpicture}\;
}
%%

%%
% Affichage des threads
\makeatletter
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  save picture id/.code={%
    \edef\pgf@temp{#1}%
    \immediate\write\pgfutil@auxout{%
      \noexpand\savepointas{\pgf@temp}{\pgfpictureid}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@#1}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  }
}

\def\savepointas#1#2{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
}

\def\tmk@labeldef#1,#2\@nil{%
  \def\tmk@label{#1}%
  \def\tmk@def{#2}%
}

\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
  \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
  \pgfsys@getposition{\pgfpictureid}\save@this@pic%
  \pgf@process{\pgfpointorigin\save@this@pic}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@process{\pgfpointorigin\save@orig@pic}%
  \advance\pgf@x by -\pgf@xa
  \advance\pgf@y by -\pgf@ya
  }%
}


%\newcommand\tikzmark[2][]{%
%\tikz[remember picture with id=#2] #1;}
\makeatother
%%


\newcommand{\FA}{\mathcal{A}_{\mathit{fresh}}}
\newcommand{\Addr}{\mathit{Addr}}
\newcommand{\interp}[1]{\llbracket #1 \rrbracket}
\newcommand{\lfp}{\mathsf{lfp}}
\newcommand{\inv}{\ensuremath{\C{I}}}
\newcommand{\gfp}{\mathsf{gfp}}
\newcommand{\fv}{\mathsf{fv}}
\newcommand{\card}{\mathsf{card}}
\newcommand{\weight}[1]{\mathsf{w}(#1)}
\newcommand{\visW}[1]{\mathsf{vw}(#1)}
\newcommand{\visP}[1]{\mathsf{vp}(#1)}
\newcommand{\hiddenP}[1]{\mathsf{hp}(#1)}
\newcommand{\visO}[1]{\mathsf{vo}(#1)}
\newcommand{\defname}[1]
{\textbf{\emph{#1}}}%{\emph{#1}}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}

\newcommand{\MALL}{\ensuremath{\mathsf{MALL}}\xspace}
\newcommand{\MLL}{\ensuremath{\mathsf{MLL}}\xspace}
\newcommand{\muMALL}{\ensuremath{\mu\mathsf{MALL}}\xspace}
\newcommand{\muSMALL}{\ensuremath{\mu\mathsf{SMALL}}\xspace}
\newcommand{\mupSMALL}{\ensuremath{\mu\mathsf{pSMALL}}\xspace}
\newcommand{\muMLL}{\ensuremath{\mu\mathsf{MLL}}\xspace}
\newcommand{\muMALLi}{\ensuremath{\mu\mathsf{MALL}^\infty}\xspace}
\newcommand{\muMALLo}{\ensuremath{\mu\mathsf{MALL}^\omega}\xspace}
\newcommand{\muSMALLi}{\ensuremath{\mu\mathsf{SMALL}^\infty}\xspace}
\newcommand{\muSMALLo}{\ensuremath{\mu\mathsf{SMALL}^\omega}\xspace}
\newcommand{\mupSMALLi}{\ensuremath{\mu\mathsf{pSMALL}^\infty}\xspace}
\newcommand{\mupSMALLo}{\ensuremath{\mu\mathsf{pSMALL}^\omega}\xspace}
\newcommand{\muMLLi}{\ensuremath{\mu\mathsf{MLL}^\infty}\xspace}
\newcommand{\muMLLo}{\ensuremath{\mu\mathsf{MLL}^\omega}\xspace}
\newcommand{\muMLLim}{\ensuremath{\mu\mathsf{MLL}_\mathsf{m}^\infty}\xspace}
\newcommand{\muMALLit}{\ensuremath{\mu\mathsf{MALL^\infty_\tau}}\xspace}
\newcommand{\muSMALLit}{\ensuremath{\mu\mathsf{SMALL^\infty_\tau}}\xspace}
\newcommand{\muMLLit}{\ensuremath{\mu\mathsf{MLL^\infty_\tau}}\xspace}
\newcommand{\muMALLim}{\ensuremath{\mu\mathsf{MALL}_\mathsf{m}^\infty}\xspace}
\newcommand{\muSMALLim}{\ensuremath{\mu\mathsf{SMALL}_\mathsf{m}^\infty}\xspace}
\newcommand{\encc}[1]{[#1]}
\newcommand{\Next}{\bigcirc}

% connecteurs logiques
\newcommand{\with}{\binampersand}
\newcommand{\parr}{\bindnasrepma}
\newcommand{\tr}{Tr}
\newcommand{\tensor}{{\otimes}}
\newcommand{\plus}{{\oplus}}
\newcommand{\llimp}{\multimap}
%\newcommand{\llone}{1}
\newcommand{\llzero}{\mathbf{0}}
\newcommand{\llone}{\mathbf{1}}
\newcommand{\shiftdown}{{\downarrow}}
\newcommand{\shiftup}{{\uparrow}}
\newcommand{\lrule}[1]{\texttt{(#1)}}
\newcommand{\dai}{{\footnotesize\maltese}}
% informatique, automates
\newcommand{\trans}[2]{\xrightarrow[\,#2\,]{\,#1\,}}
\newcommand{\dom}{\TT{Dom}}
\newcommand{\Ai}{\mathtt{i}}
\newcommand{\Al}{\mathtt{l}}
\newcommand{\Ar}{\mathtt{r}}
\renewcommand{\phi}{\varphi}

%%
% Inférences
%%
\newcommand{\mkrule}[1]{{\scriptsize\ensuremath{\mathsf{(#1)}}}\xspace}

\newcommand\rweaknatl{\mkrule{WNat_l}}
\newcommand\rax{\mkrule{Ax}}
\newcommand\rcut{\mkrule{Cut}}
\newcommand\rfrozencut{\mkrule{Cut^{\text{\ding{100}}}}}
%\newcommand\rfrozencut{\mkrule{Cut^\Snowflake}}
\newcommand\rdaimon{\mkrule{\daimon}}
\newcommand\rnext{\mkrule{\Next}}
\newcommand\rweak{\mkrule{W}}
\newcommand\rweakl{\mkrule{W_l}}
\newcommand\rweakr{\mkrule{W_r}}
\newcommand\rnegl{\mkrule{Neg_l}}
\newcommand\rnegr{\mkrule{Neg_r}}
\newcommand\rdisjl{\mkrule{\vee_{l}}}
\newcommand\rdisjr{\mkrule{\vee_{r}}}
\newcommand\rdisj{\mkrule{\vee}}
\newcommand\rbot{\mkrule{\bot}}
\newcommand\rconjl{\mkrule{\wedge_{l}}}
\newcommand\rconjr{\mkrule{\wedge_{r}}}
\newcommand\rconj{\mkrule{\wedge}}
\newcommand\rtop{\mkrule{\top}}
\newcommand\rsigma{\mkrule{\sigma}}
\newcommand\rsigmal{\mkrule{\sigma_{l}}}
\newcommand\rsigmar{\mkrule{\sigma_{r}}}
\newcommand\rmul{\mkrule{\mu_{l}}}
\newcommand\rmur{\mkrule{\mu_{r}}}
\newcommand\rmu{\mkrule{\mu}}
\newcommand\rnul{\mkrule{\nu_{l}}}
\newcommand\rnur{\mkrule{\nu_{r}}}
\newcommand\rnu{\mkrule{\nu}}
\newcommand\rnui{\mkrule{\nu I}}
\newcommand\rnue{\mkrule{\nu E}}
\newcommand\rfuncto{\mkrule{Functo}}
\newcommand\rrightarrow{\mkrule{\rightarrow}}
\newcommand\rs{\mkrule{S}}
\newcommand\rb{\mkrule{B}}
\newcommand\rt{\mkrule{\tau}}
\newcommand\rtp{\mkrule{\tau'}}
\newcommand\rN{\mkrule{r_N}}
\newcommand\rassumption{\mkrule{A}}
\newcommand\runfoldr{\mkrule{Unfold_r}}
\newcommand\runfoldl{\mkrule{Unfold_l}}
\newcommand\rwith{\mkrule{\with}}
\newcommand\rwithl{\mkrule{\with_1}}
\newcommand\rwithr{\mkrule{\with_2}}
\newcommand\rwithi{\mkrule{\with_i}}
\newcommand\rparr{\mkrule{\parr}}
\newcommand\rotimes{\mkrule{\otimes}}
\newcommand\rotimesl{\mkrule{\otimes_l}}
\newcommand\rotimesr{\mkrule{\otimes_r}}
\newcommand\rtensor{\mkrule{\otimes}}
\newcommand\roplus{\mkrule{\oplus}}
\newcommand\roplusl{\mkrule{\oplus_1}}
\newcommand\roplusrl{\mkrule{\oplus_{r1}}}
\newcommand\roplusrr{\mkrule{\oplus_{r2}}}
\newcommand\roplusr{\mkrule{\oplus_2}}
\newcommand\roplusi{\mkrule{\oplus_i}}
\newcommand\roplusj{\mkrule{\oplus_j}}
%\newcommand\rone{\mkrule{\llone}}
\newcommand\rone{\mkrule{\llone}}
\newcommand\rdai{\mkrule{\dai}}
\newcommand\rmcut{\mkrule{mcut}}
\newcommand\rmcutone{\mkrule{mcut_1}}
\newcommand\rmcuttwo{\mkrule{mcut_2}}
\newcommand\rmcutpar{{\scriptsize\ensuremath{\mathsf{mcut(\iota, \perp\!\!\!\perp)}}}\xspace}
\newcommand\mcutred[1]{\underset{#1}{\longrightarrow}}

\newcommand\red{\rightarrow}

%\newcommand\actl{\mathtt{l}}
%\newcommand\actr{\mathtt{r}}
%\newcommand\acti{\mathtt{i}}

